A Hamilton Cycle in the $k$-Sided Pancake Network

We present a Hamilton cycle in the $k$-sided pancake network and four combinatorial algorithms to traverse the cycle. The network's vertices are coloured permutations $\pi = p_1p_2\cdots p_n$, where each $p_i$ has an associated colour in $\{0,1,\ldots, k{-}1\}$. There is a directed edge $(\pi_1,\pi_2)$ if $\pi_2$ can be obtained from $\pi_1$ by a "flip" of length $j$, which reverses the first $j$ elements and increments their colour modulo $k$. Our particular cycle is created using a greedy min-flip strategy, and the average flip length of the edges we use is bounded by a constant.

==> loop-free.tex <==
\subsection{Loop-free Generation of the Flip Sequence $\SEQQ^k_{n}$}

Based on the recursive definition of the flip sequence  $\SEQQ^k_{n}$ given in \red{(?)},  Algorithm~\ref{alg:iter} will generate $\SEQQ^k_{n}$ in a loop-free manner.  The algorithm generalizes a near identical algorithm presented by Zaks for non-coloured permutations~\cite{zaks}.  The next flip size $x$ is computed using an array of counters $c_1,c_2,\ldots ,c_{n+1}$ initialized to 0, and an array of flip sizes $f_1,f_2, \ldots , f_{n+1}$ with each $f_i$ initialized to $i$.  For a formal proof of correctness, we invite the readers to see the simple inductive proof for the non-coloured case in~\cite{zaks}, and note the primary changes required to generalize to coloured permutations are in handling of the minimum allowable flip sizes (when $k=1$, the smallest allowable flip size is 2) corresponding to lines 4-5 and adding a factor of $k$ to line 7.  
%A complete C implementation of this iterative generation approach is provided in the appendix.

%-----------------------
\begin{algorithm}[h]
  \caption{Loop-free generation of the flip-sequence $\SEQQ^k_{n}$ }
  \label{alg:iter}
    \small

  \begin{algorithmic}[1]

    \Procedure{FlipSeq}{} 
    
    		\State $c_1,c_2, \ldots ,c_{n+1} \gets 0,0,\ldots , 0$
		\State $f_1,f_2, \ldots , f_{n+1} \gets 1,2, \ldots , n+1$

	\Repeat

		%\State \Call{Visit}{$\mathbf{p}$}
		

	
		  \If{$k = 1$}   $x \gets f_{2}$;  \ \   $f_{2} \gets 2$
		\Else \ \ $x \gets f_{1}$;  \ \   $f_{1} \gets 1$
		\EndIf
 		 \State $c_x \gets c_x + 1$ 
  		\If{ $c_x = kx{-}1$ } 
   			 \State $c_x \gets 0$
   			 \State $f_x \gets f_{x+1}$
   			 \State $f_{x+1} \gets x+1$
 		 \EndIf 
  		\State \Call{Output}{$x$}
		
		%\State \Call{Visit}{$\mathbf{p}$}
  
		%\State $\mathbf{p} \gets \flip{j}(\mathbf{p})$ 
	\Until $x > n$ 
    \EndProcedure

  \end{algorithmic}
  


\end{algorithm}
%-----------------------



%

\begin{theorem}
The algorithm  {\sc FlipSeq} is a loop-free algorithm to generate the flip sequence  $\SEQQ^k_{n}$ one element at a time.
\end{theorem}



Since the average flip size in $\SEQQ^k_{n}$  is bounded by a constant, as determined in the previous subsection, Algorithm~\ref{alg:iter} can be modified to generate $\RecCMin{\mathbf{p}}{k}$ by initializing a permutation $\pi$ to $\mathbf{p}$, outputting the current permutation $\pi$ at the start of the {\bf repeat} loop,  and updating 
$\pi \gets \flip{x}(\pi)$ at the end of the loop instead of outputting the flip size.


\begin{corollary}
The algorithm {\sc FlipSeq}  can be modified to generate successive permutations in the listing $\RecCMin{\mathbf{p}}{k}$  in $O(1)$-amortized time.
\end{corollary}









\begin{comment}
%-----------------------
\begin{algorithm}[h]
  \caption{Iterative approach to list $\RecCMin{\mathbf{p}}{k}$ }
  \label{alg:iter}
    \small
    
      \begin{algorithmic}[1]
 \Function{\NEXT}{} \  {\bf returns}  integer  
  		\If{$k = 1$}   $x \gets f_{2}$;  \ \   $f_{2} \gets 2$
		\Else \ \ $x \gets f_{1}$;  \ \   $f_{1} \gets 1$
		\EndIf
 		 \State $c_x \gets c_x + 1$ 
  		\If{ $c_x = kx{-}1$ } 
   			 \State $c_x \gets 0$
   			 \State $f_x \gets f_{x+1}$
   			 \State $f_{x+1} \gets x+1$
  \EndIf 
  		\State  \Return $x$
\EndFunction
\end{algorithmic}

\medskip

  \begin{algorithmic}[1]

    \Procedure{IterativeGen}{$\mathbf{p}$} 

	\Repeat

		\State \Call{Visit}{$\mathbf{p}$}
		\State $j \gets$ \Call{\NEXT}{} 
		\State $\mathbf{p} \gets \flip{j}(\mathbf{p})$ 
	\Until $j > n$ 
    \EndProcedure

  \end{algorithmic}
  


\end{algorithm}
%-----------------------
\end{comment}
%If a call to \Call{\NEXT}{} s $O(1)$ time, then this algorithm will produce the respective exhaustive listing in $O(1)$ time per flip.


%






